Multilingual and Multimodal Topic Modelling with Pretrained Embeddings

This paper presents M3L-Contrast -- a novel multimodal multilingual (M3L) neural topic model for comparable data that maps texts from multiple languages and images into a shared topic space. Our model is trained jointly on texts and images and takes advantage of pretrained document and image embeddings to abstract the complexities between different languages and modalities. As a multilingual topic model, it produces aligned language-specific topics and as multimodal model, it infers textual representations of semantic concepts in images. We demonstrate that our model is competitive with a zero-shot topic model in predicting topic distributions for comparable multilingual data and significantly outperforms a zero-shot model in predicting topic distributions for comparable texts and images. We also show that our model performs almost as well on unaligned embeddings as it does on aligned embeddings.

==> COLING-2022--Arxiv--M3L Topic Modelling/ablation.tex <==
\label{sec:ablation-study}


\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/ablation-topic-num-MRR.png}
    \caption{Effect of increasing topic numbers on cross-lingual retrieval performance (MRR).}
    \label{fig:text-only-topic-numbers}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/ablation-topic-num-UAP.png}
    \caption{Effect of increasing topic numbers on text-image retrieval performance (UAP).}
    \label{fig:text-images-topic-numbers}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.55\textwidth]{figures/ablation-M3LContrast-batch-sizes-text-only.png}
    \caption{Effect of different batch sizes on M3L-Contrast trained on multilingual text data.} %Cross-lingual retrieval (MRR) is best with batch size 32. Averaged JSD between matching articles goes down with increasing batch sizes but does not result in better retrieval performance.}
    \label{fig:text-only-batch-sizes}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.55\textwidth]{figures/ablation-M3LContrast-batch-sizes-text-images.png}
    \caption{Effect of different batch sizes for M3L-Contrast trained on multilingual text \textit{and} images.} %We show text-image retrieval (UAP) with English and German as query articles. Batch size 32 is best for English while 64 is best for German. JSD between matching articles and images goes down with increasing batch sizes but does not result in better retrieval performance.}
    \label{fig:text-images-batch-sizes}
\end{figure}

\begin{table*}[t!]
\centering
\begin{tabular}{l l | r r | r r | r r}
%\Xhline{1.5pt}
\hline
\multicolumn{2}{c}{\textbf{Encoders}} & \multicolumn{2}{c}{\textbf{EN-DE text}} &  \multicolumn{2}{c}{\textbf{EN-images}} & \multicolumn{2}{c}{\textbf{DE-images}}\\
%\Xhline{1.5pt} 
%\hline
\textbf{Text} & \textbf{Image}&  \textbf{MRR$\uparrow$} & \textbf{JSD$\downarrow$} & \textbf{UAP$\uparrow$} & \textbf{JSD$\downarrow$}  & \textbf{UAP$\uparrow$} & \textbf{JSD$\downarrow$} \\
\hline 
CLIP & CLIP & {0.613} & {0.035} & \textbf{0.125} & {0.130} & {0.102} & {0.147}\\
\hline
multilingual SBERT & CLIP & \textbf{0.716} & \textbf{0.029} & {0.119} & {0.137} & \textbf{0.114} & {0.147}\\
%\hline
monolingual SBERTs & CLIP & {0.407} & {0.052} & {0.118} & \textbf{0.129} & {0.102} & \textbf{0.141}\\
%\hline
multilingual SBERT & ResNet & {0.659} & {0.028} & {0.053} & {0.160} & {0.047} & {0.167}\\
%\hline
monolingual SBERTs & ResNet & {0.347} & {0.050} & {0.053} & {0.145} & {0.052} & {0.157}\\
\hline
\end{tabular}
\caption{Effect of different encoder combinations for M3L-Contrast trained on \textbf{multilingual text and images} compared to CLIP with 100 topics.}
\label{tab:text-images-encoders}
\end{table*}


\subsection{Topic numbers}
In Figure~\ref{fig:text-only-topic-numbers} we show the models' performance on cross-lingual text retrieval (MRR) for $[25, 50, 100]$ topics. ZeroshotTM performs best for all topic numbers followed by M3L-Contrast. Figure~\ref{fig:text-images-topic-numbers} shows the results for text-image retrieval (UAP). M3L-Contrast performs best for all topic numbers while ZeroshotTM performs worst. In general, performance improves as the topic number increases.

%As can be seen from Figures~\ref{fig:text-only-topic-numbers} and~\ref{fig:text-images-topic-numbers}, the retrieval performance increases with the number of topics. %However, optimizing a topic model with retrieval objective is dangerous since that would diminish the interpretability of the model. We noticed that as the number of topics increases the more topics appear to be redundant and or spurious topics. 
%The topic coherence, measured with NPMI, usually decreases with larger topic numbers. 

\subsection{Batch sizes for M3L-Contrast}
%We experiment with different batch sizes for the M3L-Contrast model is an critical hyperparameter in contrastive learning. 
We check batch sizes $[16, 32, 64, 128]$. Figure~\ref{fig:text-only-batch-sizes} shows the effect of increasing batch sizes for M3L-Contrast trained only on multilingual articles. We find that batch size 32 is the best for the multilingual setting. We also run similar experiments with multilingual text \textit{and} images (Figure~\ref{fig:text-images-batch-sizes}). In the multimodal setting, size 32 performs the best when English articles are matched to images while 64 is best for German. This is why we used batch size 32 for our experiments with M3L-Contrast. %For the rest of our M3L-Contrast experiments, we use batch size 32. 

%Interestingly, in both cases the divergence between corresponding articles decreases as the batch size grows but it does not result in better retrieval performance. This probably indicates the general limitation of topic modelling for retrieval tasks.



\subsection{Encoder combinations for M3L-Contrast}


To show how unaligned encoders perform with M3L-Contrast, we experiment with two encoder combinations: (1) a multilingual text encoder and an unaligned image encoder; and (2) unaligned monolingual text encoders and an unaligned image encoder. For this experiment, we train M3L-Contrast with multilingual articles \textit{and} images and evaluate the models on cross-lingual retrieval and text-image retrieval. Encoder details are in the Appendix. Results are shown in Table~\ref{tab:text-images-encoders}. 

For cross-lingual text retrieval, using a multilingual encoder performs best since this model is trained specifically on multilingual texts and has a larger embedding dimension than CLIP (768 and 512, respectively). For English text-image retrieval, it is expected that CLIP is the best since the text and image embeddings are already aligned (first row). CLIP image embeddings performed better than ResNet on all measures.

It is encouraging that M3L-Contrast with unaligned text and image embeddings still outperform ZeroshotTM and ZeroshotTM-KD (compare with Table~\ref{tab:results-text-images}, top part) even though those models use aligned embeddings. This shows that contrastive learning is effective in mapping unanligned embeddings into a shared topic space and that it is not necessary to use aligned embeddings in multimodal topic modelling. 



==> COLING-2022--Arxiv--M3L Topic Modelling/conclusion.tex <==
%Training topic modelling for images for a long time has been a goal for many researchers in the area. With the advent of multimodal embeddings and neural topic modelling producing multimodal topic models has become possible without any changes in the model. ZeroshotTM---or any other neural TM that uses embeddings as an input---can be trained on textual data encoded with multimodal distributional model, such as CLIP~\cite{radford2021learning},  and then applied to images. 

%Such zero-shot approach has been used before to obtain multilingual topic models~\cite{bianchi-etal-2021-cross}. In this paper, a similar experiment was for the first time conducted in a multimodal setting, demonstrating that a zero-shot approach for topic modelling could be used across modalities.

%However, the zero-shot approach has a serious limitation since it assumes that a pretrained aligned representation model exists for the data at hand. This is not always the case, and training such a model usually requires a big parallel dataset, much bigger than datasets commonly used to train multilingual topic models. 

%Moreover, the zero-shot approach somehow diminishes one of the main purposes of topic modelling, namely its ability to describe latent semantic themes in an input collection. Since a zero-shot model is trained on a single language it would contain biases encoded in a source data collection and would map all other languages and modalities in the source thematic structure. The same holds for the knowledge-distillation approach, where one language is used to train a 'teacher' model, that is then used to train 'student' models for other languages and modalities.

We presented M3L-Contrast, a multimodal and multilingual neural topic model based on ZeroshotTM that uses pretrained document and image embeddings. M3L-Contrast is trained jointly on multilingual texts and images and does not require aligned embeddings. Since it is a \textit{multilingual} topic model it produces aligned language-specific topics. As a \textit{multimodal} topic model, it maps texts and images into a shared topic space and infers textual representations, through the topic words, of the semantic concepts present in the images. %to produce the contextualised representations that is inputted into the model and it is trained jointly on all data views presented in the collection. 

%We believe that this would make the model less prone to biases represented in a certain language and plan to investigate the model behaviour in a low-resource setting. 

%An additional advantage of M3LContrast is its ability to produce topic labels in all languages present in the training data. 

%We performed quantitative evaluations of M3L-Contrast in multilingual and multimodal settings. 
We show that in the multilingual setting, M3L-Contrast improves on PLTM, a classical multilingual topic model, and that it is competitive with ZeroshotTM in the alignment of topic distributions for comparable documents in different languages. In the multimodal setting, our model significantly improves on ZeroshotTM %(and ZeroshotTM-KD) 
in aligning comparable texts and images in the topic space. Moreover, with unaligned text and image embeddings our model still performs better than ZeroshotTM that uses aligned embeddings.

%Our results show that M3L-Contrast also significantly improves on ZeroshotTM in multimodal topic modelling. In a text-only setting it outperforms a non-neural multilingual PLTM model and demonstrates comparable performance with ZeroshotTM. 

%Thus, the advantage of joint training is important for multimodal topic modelling and less important in multilingual setting, at least for such big languages as English and German. The possible explanation for that is modality gap~\cite{ModalityGap2022}, i.e. the property of multimodal representations to keep different modalities apart in the representation space, that makes zero-shot approach less efficient.

%As far as we know, the M3L-Contrast is the first joint neural multilingual and multimodal topic model. %Potential applications of this model include topic-aware image clustering, image recommendations, and mult imodal search. 
Our proposed architecture can easily be extended to include other modalities beyond image and text. We also believe that M3L-Contrast will be useful in a low-resource setting, where aligned embeddings can be difficult to obtain.

==> COLING-2022--Arxiv--M3L Topic Modelling/experiments.tex <==
\subsection{Dataset}
We run experiments on our proposed model on a dataset of aligned English and German Wikipedia articles and images. We take aligned articles from the Wikipedia Comparable Corpora\footnote{\url{https://linguatools.org/tools/corpora/wikipedia-comparable-corpora/}} and align them with images from the Wikipedia-based Image Text dataset (WIT)~\cite{srinivasan2021wit} \footnote{\url{https://github.com/google-research-datasets/wit}}. We use articles instead of the image descriptions in WIT because topic models are designed for full documents, rather than snippets of text. 

We randomly select 20,000 tuples for training. Since articles can be associated with more than one image and we want fixed-size tuples during training, we randomly select one image per article pair. For testing, we randomly select 1,000 article pairs. We consider \textit{all} images aligned with the paired articles, which results in 3,278 unique tuples in the test set.  

\subsection{Evaluation}
We evaluate M3L-Contrast in the multilingual setting and the multimodal setting, separately. In the multilingual case we train M3L-Contrast on multilingual articles \textit{without} images and for the multimodal case on the multilingual articles \textit{and} images.

We want document-topic distributions for multilingual articles and images from the same tuple to be similar to each other 
\textit{and} distinct from other examples. Thus, we evaluate the alignment of topic distributions using retrieval tasks.\footnote{We are aware that topic distributions do not outperform raw embeddings in retrieval tasks but the point of this evaluation is not to improve cross-lingual or cross-modal retrieval but to evaluate the alignment of the topic distributions.}

Texts and images are fed one at a time to their own language-specific and modality-specific inference networks to obtain topic distributions. For the multilingual setting, we match an English article to the most similar German article in terms of the Jensen-Shannon divergence (JSD) between their respective document-topic distributions. For the multimodal setting, we match English articles to images and German articles to images, separately. We use mean reciprocal rank (MRR) to measure text retrieval performance and uninterpolated average precision~\cite[UAP,][]{manning1999topics} to measure text-image retrieval performance because multiple images can be associated with an article.

We also report the averaged JSD between the topic distributions for all data pairs from the same tuple. Lastly, we compute language-specific topic coherences with respect to the training data using normalised pointwise mutual information~\cite[NPMI,][]{roder2015exploring}\footnote{Computed using the Gensim library~\cite{rehurek2010software}.}. 

\subsection{Baselines}
%\begin{itemize}
    %\item 
    ~~~\textbf{PLTM}~\cite{mimno2009polylingual} We implement PLTM with Gibbs sampling.
 
    %\item 
    \textbf{ZeroshotTM}~\cite{bianchi-etal-2021-cross} We train separate models on the English and German articles using the authors' original implementation.\footnote{\url{https://github.com/MilaNLProc/contextualized-topic-models}}
 
    %\item 
    \textbf{ZeroshotTM-KD}~\cite{pivovarova2021visual} We adapt ZeroshotTM for multilingual or multimodal settings using knowledge distillation~\cite{hinton2015distilling}. This method uses the parameters learned by the teacher model as priors for the student. We train four separate teacher-student pairs: (1) Model trained on English articles as teacher, German as student; (2) German articles as teacher, English as student; (3) English articles as teacher, images as student; and (4) German articles as teacher, images as student.
%\end{itemize}

\subsection{Configurations}
We report the performance of the neural topic models using CLIP~\cite{radford2021learning} as our multimodal multilingual encoder for a fair comparison.\footnote{ \textit{clip-ViT-B-32} for images and  \textit{clip-ViT-B-32-multilingual-v1} for texts.} CLIP is a pretrained vision-language model trained on web-scale data that encodes text and images into a common embedding space. We train all models with 100 topics for 100 epochs. Other hyperparameters are discussed in the Appendix. We use batch size 32 for M3L-Contrast. In Section~\ref{sec:ablation-study} we show the performance of M3L-Contrast for different encoder combinations (aligned and unaligned), different batch sizes and topic numbers.

%It has been shown that in document retrieval topic modelling does not outperform embedding-based models~\cite{zosa-etal-2020-comparison} and the same results holds for text-image matching~\cite{pivovarova2021visual}. We do not propose any document matching methods in this paper but rather use this task as a way to measure model consistency across multiple data views.




==> COLING-2022--Arxiv--M3L Topic Modelling/impact.tex <==
\subsection*{Potential impact and risks}
Our models are currently for research purposes only. We do not advise that it be used in production settings. Our models might associate images of people and objects with negative and insensitive stereotypes if the training data has these associations. Since we use CLIP to encode texts and images in our experiments, our models might also perpetuate the harmful stereotypes found in the CLIP training data discussed in~\cite{birhane2021multimodal}. The same issue applies to the other pretrained encoders we use in our experiments.

%Furthermore, our models might associate images with topics that are inconsistent with the image content. Therefore these outputs must be used with caution in applications such as image tagging and image clustering.

%\subsection*{Intended use of datasets}
%The Wikipedia Image Text (WIT) dataset is for multimodal multilingual models and tasks. The Wikipedia Comparable Corpora is for multilingual/cross-lingual tasks. Since we link the images in WIT with full articles from the Comparable Corpus using article titles, we want to emphasize that these linked articles and images should not be used outside of research settings because we cannot guarantee that all the article-image associations are correct.

==> COLING-2022--Arxiv--M3L Topic Modelling/introduction.tex <==
Topic modelling is an unsupervised method initially designed for text data that extracts latent themes in documents through the co-occurrence statistics of the words in the documents. In most probabilistic topic models, a topic is a distribution over a vocabulary and a document is a distribution over topics~\cite{blei2003latent}. Multilingual topic models extend basic topic models for multilingual data by jointly training on multiple languages~\cite{mimno2009polylingual,hao2018learning}. These models learn aligned language-specific topics and have been used in different cross-lingual applications such as multilingual news clustering~\cite{de2009cross} and comparing discourses from different cultures in news and social media~\cite{shi2016detecting,gutierrez2016detecting}.

Most topic models are designed for textual data but there is also a rich body of work on applying topic modelling to images resulting in multimodal topic models~\cite{barnard2003matching,feng2010visual,roller2013multimodal}. These models use natural language supervision to improve the semantic representation of images. Augmenting topical information from text with topic information from visual inputs also produces better semantic representations of words.

Neural topic models have been proposed to improve on classical topic models and have resulted in models that are more computationally efficient and produces more coherent topics~\cite{srivastava2017autoencoding}. Moreover, the neural topic modelling framework has given rise to models that take advantage of information from external sources such as word embeddings~\cite{dieng2020topic} and contextualised language models~\cite{bianchi-etal-2021-pre,bianchi-etal-2021-cross,hoyle2020improving,mueller2021fine}.

In this work, we present a novel neural multilingual \textit{and} multimodal topic model that takes advantage of pretrained document and image embeddings to abstract the complexities between languages and modalities. Our work is based on the contextualized topic model~\cite[CTM,][]{bianchi-etal-2021-pre,bianchi-etal-2021-cross}, a family of topic models that uses contextualized document embeddings as input. 

We show that while ZeroshotTM~\cite{bianchi-etal-2021-cross}, a cross-lingual variant of CTM, can predict relevant topic distributions of documents in languages it has not seen during training, this ability does not transfer well to unseen modalities (e.g. images). Moreover, since ZeroshotTM only sees monolingual data, it produces monolingual topics that are inferred from documents in a single language. This approach does not take into account possible biases in worldviews that are hidden in different languages. %It has also been shown that zero-shot modelling tends to assign documents from an unseen language to only a small subset of available topics~\cite{mueller2021fine}.

Our approach, which we refer to as M3L-Contrast, trains jointly on multilingual texts and images with a contrastive objective. We show that our model produces better topic distributions for comparable texts and images compared to ZeroshotTM even with unaligned embeddings and our model also improves on a classical multilingual topic model for comparable multilingual data. The main contributions of this work are:
\begin{enumerate}[nosep]
    \item  We present a neural multimodal \textit{and} multilingual topic model for comparable data that maps images and texts into a shared topic space;
    \item we show that contrastive learning is effective in mapping embeddings from unaligned encoders into a shared topic space \textit{and} improves on the alignment of aligned embeddings; 
    \item we present a multilingual topic model for comparable multilingual data that uses pretrained embeddings and improves on a classical topic model for comparable data.\footnote{Our code is available at \url{https://github.com/ezosa/M3L-topic-model}}
    %\item We show that joint contrastive training helps produce better topic representation, while taking into account potential differences in worldviews hidden in different data views.
\end{enumerate}







==> COLING-2022--Arxiv--M3L Topic Modelling/models.tex <==
\subsection{Neural multilingual topic model}
\label{sec:models-multilingual}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/m3l-contrast-new2.png}
    \caption{Proposed M3L-Contrast topic model. (a) Multilingual topic model with language-specific encoders and inference networks; (b) Extension to the multimodal setting. The loss function is detailed in Equation~\ref{eq:loss-m3l-contrast}.}
    \label{fig:archi-m3l-contrast}
\end{figure}

We first propose a neural multilingual topic model for comparable multilingual data that uses pretrained document embeddings. Our multilingual model is based on ZeroshotTM~\cite{bianchi-etal-2021-cross}, a zero-shot cross-lingual topic model. However, we are not aiming for a zero-shot model. Instead, our model infers aligned \textit{language-specific topics} for each language present in the dataset. Moreover, our approach does not require the pretrained document embeddings to be aligned beforehand. This property makes it advantageous in settings where a multilingual encoder that includes our desired language might not exist such as in low-resource settings.

Figure~\ref{fig:archi-m3l-contrast}(a) shows the multilingual model architecture. The model uses independent inference networks for each language. To align language-specific topics, the model minimizes the Kullback-Leibler (KL) divergence between the topic distributions of comparable documents from different languages and, in addition, uses a contrastive loss to map similar instances close to each other in the topic space and keep non-related instances apart.  

For each tuple of aligned documents in the comparable multilingual dataset, we encode the documents from each language using their own separate encoders (whether aligned or non-aligned) and then the embeddings are passed to language-specific inference networks that infers the mean, $\mu$, and variance, $\sigma^2$, of the Gaussian distribution from which we sample latent document-topic distributions. At this point, the languages are independent of each other and have not yet shared any information.  

After sampling topic distributions for each document, we induce a shared topic space by minimizing the pairwise KL divergence between the language-specific distributions whose parameters are estimated from their own inference network. We also add a contrastive objective so that aligned examples are kept away from other examples in the topic space. 
We use InfoNCE~\cite{van2018representation} as our contrastive loss. The positive pairs are all possible combinations of document pairs from the same tuple and negative pairs are all other pairs of documents from different tuples within a batch. For instance, for a comparable dataset with two languages and batch size $N$, we would have $N$ positive pairs and $N^2-N$ negative pairs per batch. For three languages, that would be $3N$ positive pairs and $3(N^2-N)$ negative pairs, etc.
% (n choose 2) = n! / (2 (n-2)!)

Thus, the loss consists of the three components: the reconstruction loss; the KL divergence between topic distributions; and the contrastive loss. %that ensures that pairs from the same tuple have similar topic distributions while pairs from different tuples are dissimilar in the topic space. 
Formally, the loss function is written as:
\begin{align}
\mathcal{L} & = \sum_{l=0}^{L} \mathbb{E}_{q}[w^{\top} \log(\text{softmax}(\beta_{l}\theta_{d}))] - \nonumber \\
& \sum_{\substack{a,b=0\\a \neq b}}^{n} \mathbb{KL}(p(\theta_{i}^{a} | x_{i}^{a}) || q(\theta_{i}^{b} | x_{i}^{b})) - \nonumber \\ 
& s \sum_{\substack{a,b=0\\a \neq b}}^{n} \log \frac{\exp( (\theta_{i}^{a} \cdot \theta_{i}^{b}) / \tau)}{ \sum_{j=0}^{N} \sum_{c,d=0}^{n} \exp( (\theta_{i}^{c} \cdot \theta_{j}^{d}) / \tau)}    
\label{eq:loss-m3l-contrast}
\end{align} 

The first term is the sum of the bag-of-words (BoW) reconstruction losses of each language in the corpus. %$w_d$ is the BoW representation of document $d$ for language $l$, $\beta_{l}$ is topic-term matrix for language $l$ and $\theta_d$ is the sampled topic representation for document $d$. 
We refer the reader to~\cite{srivastava2017autoencoding} for further details on the reconstruction loss.

The second term is the sum of the KL divergences between the language-specific document distributions, $p()$ and $q()$, whose mean and variance are estimated from language-specific inference networks; $\theta$ refers to the sampled topic representation of a document in a tuple where $i$ is the tuple index, $a$ and $b$ are the indices of the documents inside the tuple and $n$ is the size of the tuple. Lastly, $x$ refers to a document embedding.    

The third term is the InfoNCE loss where $(\theta_{i}^{a} \cdot \theta_{i}^{b})$ are positive pairs (they belong to the same tuple) and $(\theta_{i}^{c} \cdot \theta_{j}^{d})$ are negative pairs (they are from different tuples). $N$ is the batch size, $\tau$ is the temperature and $s$ is a constant to give additional weight to the contrastive loss.

\subsection{Extension to multimodal setting}
\label{sec:models-multimodal}
We now extend the proposed multilingual topic model to the \textit{multimodal} setting. Figure~\ref{fig:archi-m3l-contrast}(b) shows the architecture of the proposed multilingual \textit{and} multimodal topic model.  

We can think of the multimodal case as a generalization of the multilingual model. The loss function in Equation~\ref{eq:loss-m3l-contrast} remains essentially the same. Since a BoW representation is not available for images, the reconstruction loss is computed only on texts and the first loss term is unchanged. In the second term of the loss function, $x$ can be a document \textit{or} image embedding and $\theta$ is the sampled topic distribution for that embedding. 

Since the document or image embeddings abstract the modality of the data, the topic distributions are now modality-agnostic. Thus, the third term is also unchanged, except for the tuple size $n$. A multimodal dataset with one language and one image view would have $N$ positive and $N^2-N$ negative pairs, the same as in the bilingual case. For two languages \textit{and} one image, we would have $3N$ positive pairs and $3(N^2-N)$ negative pairs, as in the trilingual case. 

We refer to our proposed topic model as \textbf{M3L-Contrast} for \textit{multimodal multilingual (M3L) topic model with contrastive learning}.




==> COLING-2022--Arxiv--M3L Topic Modelling/related_work.tex <==
\subsection{Neural topic models}
Neural topic models (NTMs) refer to a class of topic models that use neural networks to estimate the parameters of the topic-word and document-topic distributions. Using a variational autoencoder (VAE) to map documents into latent topic spaces was proposed by \citet{srivastava2017autoencoding} and demonstrated in the ProdLDA model that exhibited better topic coherences and faster training than classical models. This has led to other VAE-based topic models that can incorporate information from external sources such as the Embedded Topic Model~\cite{dieng2020topic} which uses pretrained word embeddings, the Contextualised Topic Model~\cite{bianchi-etal-2021-pre} which uses contextualised embeddings and the BERT-based Autoencoder as Teacher~\cite{hoyle2020improving} model that distills large language models to improve topic coherence. %Aside from VAEs, other NTMs use Wasserstein autoencoders~\cite{nan-etal-2019-topic} and generative adversarial networks~\cite{wang2019atm,nguyen2021contrastive}.


%Though these models use distributed representations as an input and potentially can leverage multimodal embeddings, such as CLIP, to produce a topic distribution for an image, we are unaware of any previous work that actually performed such experiments. Thus, our paper is the first that demonstrates that multimodal topic modelling can be based on distributed image representations. 
%from BERT-like models and the BERT-based Autoencoder as Teacher (BAT) model that uses knowledge distillation to learn topics from parameter-rich models~\cite{hoyle-etal-2020-improving}. 
%Other NTMs use Wasserstein autoencoders~\cite{nan-etal-2019-topic} and generative adversarial networks~\cite{wang2019atm,nguyen2021contrastive} 

%Generative adversarial networks (GAN) have also been proposed as another method for inferring topic distributions. The Adversarial Topic Model~\cite{wang2019atm} is the first such method in this family and recently, an extension of ATM was proposed with a more principled approach to negative sampling and using contrastive loss to train the model~\cite{nguyen2021contrastive}. %The GAN consists of the Generator, which samples document-word distribution from the current state of the model and the Discriminator, which have to distinguish these generated distributions from those obtained from real documents. As the Generator learns to "deceive" the Discriminator, the model distributions becomes closer to the underlying distribution in the data. Recently, an extension of ATM has also been proposed. This method uses a more principle approach to negative sampling and uses contrastiive learning to train the model.
    
\subsection{Multilingual topic models}
Multilingual topic models infer aligned language-specific topics from a multilingual dataset. To align topics across languages, some degree of supervision is required to establish the link between the languages. In most cases, the languages are linked either at a word level or at a document level~\cite{hao2020empirical}. Models that use word-level supervision require a translation dictionary to link words from different languages~\cite{jagarlamudi2010extracting,hao2018learning,yang2019multilingual}. Document-level supervision requires a comparable dataset where a document in one language is linked to a thematically similar document in another language~\cite{mimno2009polylingual,de2009cross}. %These models have been used to compare issues and opinions across different communities on the Internet and social media~\cite{shi2016detecting,gutierrez2016detecting}.

The Polylingual Topic Model \cite[PLTM,][]{mimno2009polylingual} is widely-used classical multilingual topic model for comparable data. To our knowledge, the Neural Multilingual Topic Model~\cite{wu2020learning}, a model that uses word-level supervision, is the only neural multilingual topic model so far. ZeroshotTM~\cite{bianchi-etal-2021-cross}, while not a multilingual model, is capable of zero-shot cross-lingual topic inference: it can predict topic distributions for documents in unseen languages if the model is trained on embeddings from a multilingual encoder.  However, ZeroshotTM requires \textit{aligned} embeddings for zero-shot topic modelling. 


\subsection{Multimodal topic models} 
Multimodal topic models use data from different modalities %, other than text, 
to infer topics. The most popular pairing is texts and images. % because they tend to occur together and complement each other. 
Some text-and-image topic models use labelled image datasets to learn natural language representations of images using a supervised topic modelling approach~\cite{barnard2003matching,zheng2014topic}. Other models extract `visual words' from images using image feature extractors such as SIFT and images are represented as a bag of `visual words' in the same manner that documents are represented as a bag of textual words~\cite{feng2010visual,virtanen2012factorized,roller2013multimodal}.
\cite{an2020multimodal} trained visual and textual topic models from neural network representations for multimodal depression detection but does not map text and images into the same topic space.


\subsection{Contrastive learning} 
Contrastive learning is a self-supervised technique that uses different views of the same data to learn better data representations~\cite{jaiswal2021survey,liu2021self}. In contrastive training the goal is to minimize the distance between positive samples while separating them from negative samples.  Contrastive training is popular in multimodal settings such as web-scale text-image alignment~\cite{radford2021learning,jia2021scaling}, audio-visual alignment~\cite{khorrami2021evaluation} and biomedical imaging~\cite{zhang2020contrastive}.

In neural topic modelling, contrastive learning has recently been used to improve on the Adversarial Topic Model~\cite{wang2019atm} by adding a contrastive objective to the training loss and taking a more principled approach to sampling positive and negative samples~\cite{nguyen2021contrastive}. %Another example is~\cite{hoyle2020improving}, which used knowledge distillation to produce close topic distributions from bag-of-word and contextualized representations.

 %In this work, we use a contrastive learning objective during topic inference to improve the mapping of document-image pairs in the induced topic space.
%
%There were only few previous attempts to apply contrastive learning to neural topic modelling. \cite{nguyen2021contrastive} used contrastive learning to improve on the Adversarial TM by adding a contrastive objective to the training loss and taking a more principled approach to sampling positive and negative samples. In this case contrastive training was used to find the most difficult training examples. This model is monolingual. %though it is different from our approach both in model architecture---they use ATM as a backbone network while our model is an extension of CTM---and setting, since their model is monolingual.
%
%% This model is monolingual, so words and embeddings are derived from the same data view.
%
%In both cases the training results in a single topic model. In the case of M3LContrast, contrastive training results in a several topic models---one for each data view---that can be used independently during inference.
%
%
%The difference between previous work on joint image-and-text representation learning and our work is the same as between training embeddings and topic modelling in general: while embeddings allows to map any input object to a certain position in a highly multidimentional space, topic model provides an information about a content structure of  the input collection by mapping the data into a relatively small number of interpretable latent themes.
 
 %During contrastive training, different parts of the model take as an input different data views and output their representations. The loss function is based on the distance between these representations: different views on the same data item should result in close representations in the output space.
    
% %The key issue in this setting is to prevent \textit{model collapse}, i.e. outputting the same representation for all data items. The main approach to avoid collapse is to use negative samples~\cite{chopra2005learning,gutmann2010noise,schroff2015facenet}, though it is possible to use other methods, e.g. learning with momentum~\cite{grill2020bootstrap} or additional diversity constraint on the representation space~\cite{caron2020unsupervised}. 
    
% %The majority of work in the area of contrastive training is done with visual data because it is easy to obtain avarious views of the same image using data augmentation techniques like image cropping and rotation. In NLP the biggest success story of contrastive learning and data augmentation for textual data is the SentenceBERT model~\cite{reimers-gurevych-2019-sentence,thakur-etal-2021-augmented}. 
% Contrastive training is popular in multimodal settings such web-scale text and images~\cite{radford2021learning} and biomedical imaging~\cite{zhang2020contrastive}.%In the area of NLP data augmentation is less straightforward and the majority of self-supervised work is done using generative training~\cite{liu2021self}. There are few exceptions, with the biggest success story of contrastive learning and data augmentation for textual data being the SentenceBERT model~\cite{reimers-gurevych-2019-sentence,thakur-etal-2021-augmented}. %
% %Contrastive training has been also applied in different multimodal settings such web-scale text and images\cite{radford2021learning}, biomedical imaging\cite{zhang2020contrastive}.
% %Contrastive training has been also applied in a multimodal settings, e.g. to train a joint model for image and text~\cite{radford2021learning}.
    
% %In some cases, however, data augmentation is not necessary since different views on the same data are readily available. In this paper we deal with multi-lingual setting, for which multiple parallel corpora are available, as well as high-quality machine translation techniques. We also demonstrate that exact translations are not necessary since contrastive training---at least for topic modelling---could be applied using comparable corpora.



==> COLING-2022--Arxiv--M3L Topic Modelling/results.tex <==
%%% old results are in results-old.tex


\subsection{Multilingual setting}

%%%%% Text-only Evaluation start %%%%%
\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{  
\begin{tabular}{l | r r | r r}
\hline
{} & \multicolumn{2}{c}{\textbf{Coherence$\uparrow$}} & \multicolumn{2}{c}{\textbf{EN-DE text}}\\
\textbf{Model} & \textbf{EN} &  \textbf{DE} & \textbf{MRR$\uparrow$} & \textbf{JSD$\downarrow$}\\
%\Xhline{1.5pt} 
\hline 
PLTM & {0.064} & {0.044} & {0.333} & {0.067}\\
\textbf{ZeroshotTM}  & {0.113} & {0.096} & \textbf{0.997} & \textbf{0.012}\\
ZeroshotTM-KD & 0.109 & {0.092} & {0.390} & {0.081}\\ 
\hline \hline
M3L-Contrast & \textbf{0.119} & \textbf{0.097} & {0.684} & {0.036}\\ 
\end{tabular}
}
\caption{Language-specific topic coherences (NPMI) and cross-lingual retrieval peformance (MRR and JSD).}
\label{tab:results-text-only}
\end{table}
%%%%% Text-only Evaluation end %%%%%

Table~\ref{tab:results-text-only} shows the cross-lingual retrieval performance and averaged JSD of aligned articles. ZeroshotTM is the clear winner with an MRR of 0.997 and the lowest JSD. M3L-Contrast, while it does not outperform ZeroshotTM, shows encouraging results given that it has to infer twice as many topics as ZeroshotTM (bilingual case). It also outperforms PLTM, a classical multilingual topic model and the only other model, aside from M3L-Contrast, trained on multilingual articles. Moreover, M3L-Contrast also has the best topic coherences.

\subsection{Multimodal setting}

%%%%% Text and Images evaluation start %%%%%
\begin{table*}[h!]
\centering
\begin{tabular}{l | r r | r r | r r }
%\Xhline{1.5pt}
\hline
{} & \multicolumn{2}{c}{\textbf{Coherence$\uparrow$}}  & \multicolumn{2}{c}{\textbf{EN-images}} & \multicolumn{2}{c}{\textbf{DE-images}} \\
%\Xhline{1.5pt} 
%\hline
\textbf{Model} & \textbf{EN} & \textbf{DE} & \textbf{UAP$\uparrow$} & \textbf{JSD$\downarrow$}  & \textbf{UAP$\uparrow$} & \textbf{JSD$\downarrow$}\\
\hline 
ZeroshotTM & {0.113} & {0.096} & {0.034} & {0.445} & {0.039} & {0.435}\\
ZeroshotTM-KD & {0.109} & {0.092} & {0.082} & {0.128} & {0.093} & {0.146}\\
\hline \hline
\textbf{M3L-Contrast} & \textbf{0.122} & \textbf{0.097} & \textbf{0.125} & \textbf{0.130} & \textbf{0.102} & \textbf{0.147}\\
\end{tabular}
\caption{Language-specific topic coherences (NPMI) and text-image retrieval performance (UAP). JSD is the averaged JS divergence between topic distributions of aligned articles and images. Only M3L-Contrast is jointly trained on \textbf{multilingual articles and images}.}
\label{tab:results-text-images}
\end{table*}
%%%%% Text and Images evaluation end %%%%%

Table~\ref{tab:results-text-images} shows the results for text-image matching. M3L-Contrast performs the best with UAP of 0.125 and 0.102 for matching English and German articles to images, respectively, and has the lowest JSDs. In a reversal of the results for cross-lingual retrieval, ZeroshotTM performs the worst with the lowest UAP scores and highest JSDs. ZeroshotTM-KD only slightly outperforms ZeroshotTM, indicating that the success of M3L-Contrast can be attributed to \textit{joint} training and cannot be achieved with the teacher-student sequential training scheme.

These results indicate that ZeroshotTM without any modifications is not suitable for multimodal settings. One likely reason is that multimodal encoders like CLIP suffer from the so-called `modality gap' where embeddings for different modalities are mapped to separate regions in the embedding space \cite{ModalityGap2022}. %Our results show that we can alleviate the modality gap in multimodal topic modelling by adding a contrastive objective during training. %to encourage similar examples to be mapped closer to each other in the topic space and different examples to be mapped farther apart. %Elaine: Better not say this because the Modality Gap paper says that contrastive learning actually preserves this gap

Our results also indicate that for a joint multimodal and multilingual neural topic model, it could be beneficial to use a hybrid model that uses  separate inference networks for different modalities and a shared network for the same modality. We leave this for future work.

\subsection{Error analysis}
%%%%% Examples start %%%%%
\begin{table*}[ht!]
\begin{center}
\begin{tabular}{r p{2.8cm} | p{2.2cm} | p{2.3cm} | p{2.3cm}}
    \hline
    {} & {} & \textbf{EN article} & \textbf{DE article} & \textbf{Image}\\
    \hline\hline
    \multicolumn{5}{c}{Article title: \textbf{Capsicum pubescens}} \\
    \hline
    \multirow{6}{*}{\includegraphics[width=0.2\textwidth]{figures/Capsicum_pubescens_Rocoto.JPG}} & \textbf{ZeroshotTM} & {\textbf{21:} plant, leaves, flowers, tall} & {\textbf{31:} bird, south, america, species} & {\textbf{67:} university, library, museum, research}\\
    & \textbf{\textbf{ZeroshotTM-KD} \textit{(EN teacher)}} & \textbf{44: } plant, leaves, flowers, plants, genus & - & \textbf{44: } plant, leaves, flowers, plants, genus \\
    & \textbf{M3L-Contrast} & {\textbf{65:} plant, plants, leaves, flowers} 
    & {\textbf{65:} beschreibung (\textit{description}), pflanzen (\textit{plant}), selten 
    (\textit{rare}), stehen (\textit{stand})}
    &{\textbf{65:} plant, plants, leaves, flowers}\\
    \hline
    \hline
    \multicolumn{5}{c}{Article title: \textbf{Microexpression}/\textbf{Mikroexpression}} \\
    \hline
    \multirow{5}{*}{\includegraphics[width=0.25\textwidth]{figures/Universal_emotions7.JPG}} & \textbf{ZeroshotTM} & {\textbf{13}: include, cause, may, cases, occur} & {\textbf{13:} include, cause, may, cases, occur} & {\textbf{9:} bishop, catholic, pope, church, roman}\\
     & \textbf{\textbf{ZeroshotTM-KD} \textit{(EN teacher)}} & \textbf{32:} blood, symptoms, disease, cell, bone & - & \textbf{69:} album, released, song, single, group \\
     %& \textbf{\textbf{ZeroshotTM-KD} \textit{DE teacher}} & - & \textbf{20:} 20 sprachen (\textit{languages}), sprache (\textit{language}), begriff (\textit{concept}), gesprochen (\textit{spoken}), menschen (\textit{people}) & \textbf{57:} film (\textit{film}), leben (\textit{dorector}), jahren (\textit{actress}), regisseur (\textit{life}), schauspielerin (\textit{years})  \\
    & \textbf{M3L-Contrast} & {\textbf{84:} theory, term, example, social, defined} & {\textbf{84:} begriff (\textit{concept}), definition (\textit{definition}), beispiel (\textit{example}), theorie (\textit{theory}), zahl (\textit{number})} & {\textbf{5:} film, award, series, actress, born}\\
    \hline
\end{tabular}
\caption{Top topics of Wikipedia article pairs and a related image. The numbers indicate the topic indices.}
\label{tab:examples}
\end{center}
\end{table*}
%%%%% Examples end %%%%%
To further investigate differences between the models we checked some examples from the test set. We show two article-image tuples and their predicted topics in~Table~\ref{tab:examples}. The table contains the top topic for the aligned English and German articles (titles shown) and an image associated with them. 

The first example article is about pepper\footnote{\url{https://en.wikipedia.org/wiki/Capsicum_pubescens}}. ZeroshotTM predicts relevant topics for the English and German articles but off-topic for the image. %Topic numbers are different, thus in this case data re-matching failed. 
ZeroshotTM-KD (a teacher model trained on English articles and a student on images) predicts a relevant topic for the English article and the image but it has not been trained on  German. M3L-Contrast predicts relevant topics for the English and German articles and the image. %and in addition provided a topic label in German.
Though the table shows English topic labels for the image, it is equally possible to produce German image labels.
%, or English labels for German texts, if this is needed to a particular application.  

In the second example, the article about microexpressions\footnote{\url{https://en.wikipedia.org/wiki/Microexpression}} is illustrated with an image of a woman presenting basic emotions. ZeroshotTM predicts slightly relevant topics for the English and German articles but off-topic for the image. ZeroshotTM-KD also predicts a relevant topic for the English article. Although the image topic is different from the topic of the article, it is still somewhat relevant in that the model may have associated images of women with pop stars. M3L-Contrast predicts relevant topics for the English and German articles. For the image, it predicts a topic about actresses likely because the image depicts a woman.

We found similar behaviour in other cases: English and German articles are usually assigned with the same topic while the image often has a different topic. In many cases M3L-Contrast finds an aligned topic for an image while the other two models fail.

%The dataset contains many images of various plants, but the microexpression is probably unique. None of the models was able to find the aligned topic for an image, though both ZeroshotTM and M3L-Contrast found aligned topics for English and German. Yet the M3LContrast topic is more relevant for the article. 


\subsection{Visualizing the topic space}

\begin{figure*}[t!]
     \centering
     \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=0.7\textwidth]{figures/topic-space-ctm-zeroshot-annotated_no_bg-big-legend.png}
        \caption{ZeroshotTM}
        \label{fig:topic-space-ctm}
     \end{subfigure}
     \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=0.7\textwidth]{figures/topic-space-m3l-contrast-annotated_no_bg-big_legend.png}
        \caption{M3L-Contrast}
        \label{fig:topic-space-m3l-contrast}
     \end{subfigure}
    \caption{tSNE visualizations of topic distributions of multilingual texts and images inferred by ZeroshotTM and M3L-Contrast, respectively. Annotations are added manually. Best viewed in color.}
    \label{fig:topic-spaces}
\end{figure*}

To investigate the structure of the multimodal multilingual topic space, we use 2D visualizations presented in Figures~\ref{fig:topic-space-ctm} and~\ref{fig:topic-space-m3l-contrast}, for ZeroshotTM and M3L-Contrast, respectively. These figures show the proximities of multilingual texts and images, represented by their predicted topic distributions, in the topic spaces induced by the respective models and mapped into two dimensions with tSNE.\footnote{These figures are available as interactive plots in the code repository of this paper.}

In Figure~\ref{fig:topic-space-ctm}---the ZeroshotTM topic space---the topic distributions of the aligned articles are very similar to their counterparts (most of the points representing English articles are hidden under the German articles). The images, however, tend to be isolated instead of being close to their textual counterparts. This supports the modality gap hypothesis and explains why ZeroshotTM performs poorly in the text-image retrieval task.

In Figure~\ref{fig:topic-space-m3l-contrast}, the topic space induced by M3L-Contrast, articles and images tend to group together in terms of \textit{themes}---exactly the behaviour we want from a topic model. No single modality or language is isolated by itself. This explains why M3L-Contrast performs better than ZeroshotTM in text-image retrieval. On the other hand, the English and German articles are not as close to each other as in ZeroshotTM. This supports our claim that joint training takes into account data from all languages and adjusts for possible discrepancies between worldviews across languages, even though this property results in worse performance in cross-lingual text retrieval.

 
